Pufferfish Privacy Mechanisms for Correlated Data

Many modern databases include personal and sensitive correlated data, such as private information on users connected together in a social network, and measurements of physical activity of single subjects across time. However, differential privacy, the current gold standard in data privacy, does not adequately address privacy issues in this kind of data. This work looks at a recent generalization of differential privacy, called Pufferfish, that can be used to address privacy in correlated data. The main challenge in applying Pufferfish is a lack of suitable mechanisms. We provide the first mechanism -- the Wasserstein Mechanism -- which applies to any general Pufferfish framework. Since this mechanism may be computationally inefficient, we provide an additional mechanism that applies to some practical cases such as physical activity measurements across time, and is computationally efficient. Our experimental evaluations indicate that this mechanism provides privacy and utility for synthetic as well as real data in two separate domains.

==> correlationDecay.tex <==
\section{Application In BN}

The Wasserstein mechanism is a reliable theoretical upper-bound of the amount of noise needed to maintain $\epsilon-$Pufferfish privacy. However, in practice, the Wasserstein distance is often not easy to compute, nor is it necessarily tight. 
\textcolor{red}{(TODO: check the approximation methods and cite here) }
Fortunately, in many real world applications, correlation between individuals often has some nice underlying graphical structure to be exploited. Specifically, in a Bayesian Network (BN), the correlation between two nodes is likely to decay as the degree of separation between the nodes increases. 

In this section, we shall first introduce a simple setting, the 
%
``genetic disease in a small town" 
problem, to show how the correlation decays with degree of separation, then show how $\epsilon$-Pufferfish privacy can be preserved in this scenario. 
We shall also show some natural generalization to the problem and \textcolor{red}{(show the performance of such mechanism on an HMM.)}

%
\subsection{Genetic-disease-in-a-small-town Problem}
Suppose there is a small town and people living there are quite related genetically. And suppose there is a genetic disease runs in one of the family, which means the disease is passed from parents to child with certain probability. Let $X_i \in \{0,1\}$ be the random variable representing the $i$-th person's condition. And edge between $X_{j}$ and $X_i$ indicates their parent-child relationship.

%

The client is interested in some general statistics about people's health condition in the small town. In the noiseless case, suppose the statistics is $\calF$, then the exact value $\calF(X_1,\dots,X_n)$ is returned. However, there can be an adversary who are trying to infer the value of some $X_i$ from the statistic. 
%
We assume the adversary knows the underlying distribution, i.e. the complete graph structure and CPTs. We, on the other hand, only knows the graph structure and \emph{some} properties of the distribution. 

To best illustrate the correlation decay phenomenon, the graph structure is set to be a chain, with the arrows heading the same direction. 
So essentially it shows the condition of a person and all his ancestors. 
Also, a directed edge $(X, Y)$ means with probability $p$, $Y$ has the same condition as $X$ does. \questionSS{I guess this is not really possible in those \{A, a\} kind of setting? The probabilities of disease-disease and normal-normal are usually not the same?}
%

Our task is to add appropriate noise such that the output $w$ satisfies the $\epsilon$-Pufferfish privacy definition. 

\subsubsection{Correlation Decay over Separation}
The states of two nodes $X, Y$ are less 'entangled' if $P(X=x|Y=y)$ is close to $1/2$ in this binary case. That is, the state of $X$ is almost a random flip.

Let $X_0$ be the root node in a chain and $X_i$ be the $i$th node downstream. Here we will show and prove a few key observations.

\begin{lemma}{(Downstream Decay)}
\begin{align*}
P(X_n = x | X_0 = x) - \frac{1}{2} = \frac{1}{2}(2p-1)^n
\end{align*}
where $p = P(X_i = x | X_{i-1} = x)$.
\end{lemma}

\begin{proof}
Recall that with probability $p$, $X_i = X_{i+1}$. 
Let $A_i = P(X_i = x | X_0 = x)$, then
\begin{equation*}
A_i = p A_{i-1} + (1-p) (1-A_{i-1}) = (2p-1)A_{i-1} + (1-p)
\end{equation*}
with boundary conditions $A_0 = 1$.

Notice that it's a linear recurrence relation which can be solved analytically. Re-arrange the equation, we can get
\begin{equation*}
A_i - 1/2 = (2p - 1)(A_{i-1} - 1/2)
\end{equation*}
Iterate this relation for $n$ times, we will get 
\begin{equation*}
A_n = \left(A_0 - \frac{1}{2}\right)(2p - 1)^n + \frac{1}{2} = \frac{1}{2}(2p-1)^n + \frac{1}{2}
\end{equation*}
\end{proof}

\corollary
$$\frac{P(X_n = x | X_0 = x)}{P(X_n = x|X_0 = \neg x)} = \frac{\frac{1}{2} + \Delta}{\frac{1}{2} - \Delta}$$
where $\Delta = \frac{1}{2} (2p-1)^n$.
\proof
Follows from the previous lemma.

If $p$ is not uniform across all edges, this phenomenon will still hold, except that $\Delta$ will shrink at a different rate. 
Corollary 4.2 is more pertinent to our privacy definition. As long as the ratio is close to 1, the adversary cannot tell much about $X_n$ given $X_0$, even $P(X_n = x|X_0 = x)$ and $P(X_n = x|X_0 = \neg x)$ are not close to $1/2$.

Can we also find an upstream decay using the same technique? No. In fact, by Bayes' Rule, $P(X_0 = x | X_n = x) = P(X_n = x | X_0 = x) P(X_0 = x) / P(X_n = x)$. When $n$ is large, $P(X_n = x | X_0 = x)$ and $P(X_n = x)$ tends to $1/2$, but this is not true for $P(X_0 = x)$. Fortunately, we can modify the notion the upstream decay to still get a useful result similar to Corollary 4.2 for the Pufferfish network, which is ultimately what we care.

\begin{lemma}{(Upstream Decay)}
\begin{align*}
\left(\frac{\frac{1}{2} - |\Delta|}{\frac{1}{2} + |\Delta|}\right)^2 \leq \frac{P(X_0 = x | X_n = x)}{P(X_0 = x | X_n = \neg x)} \leq \left(\frac{\frac{1}{2} + |\Delta|}{\frac{1}{2} - |\Delta|}\right)^2
\end{align*}
where $\Delta = \frac{1}{2} (2p-1)^n$. Moreover, 
\begin{align*}
\lim_{n \to \infty} \frac{P(X_0 = x | X_n = x)}{P(X_0 = x | X_n = \neg x)} = 1.
\end{align*}
\end{lemma}
\begin{proof}
First,
\begin{align*}
&\ P(X_n = x) \\
= &\ P(X_n = x | X_0 = x) P(X_0 = x) +
P(X_n = x | X_0 = \neg x) P(X_0 = \neg x)\\
= &\ \left(\frac{1}{2} + \Delta\right) q + \left(\frac{1}{2} - \Delta\right)(1-q)\\
= &\ \frac{1}{2} + (2q - 1)\Delta
\end{align*}
where $q = P(X_0 = x)$.\\
Then we have
\begin{align*}
R =&\ \frac{P(X_0 = x | X_n = x)}{P(X_0 = x | X_n = \neg x)}\\
=&\ \frac{P(X_n = x | X_0 = x) P(X_0 = x)P(X_n = \neg x)}{P(X_n = \neg x | X_0 = x)P(X_0 = x)P(X_n = x)}\\
=&\ \frac{P(X_n = x | X_0 = x) P(X_n = \neg x)}{P(X_n = \neg x | X_0 = x)P(X_n = x)}\\
=& \left(\frac{\frac{1}{2} + \Delta}{\frac{1}{2} - \Delta}\right) \left(\frac{\frac{1}{2} - (2q - 1)\Delta}{\frac{1}{2} + (2q - 1)\Delta}\right)
\end{align*}
If $\Delta \geq 0$, then $1 \leq R \leq \left(\frac{\frac{1}{2} + \Delta}{\frac{1}{2} - \Delta}\right)^2$.

If $\Delta < 0$, then $ \left(\frac{\frac{1}{2} + \Delta}{\frac{1}{2} - \Delta}\right)^2 \leq R\leq 1$.

Either way, the ratio is close to 1 when the separation $n$ is large because $\Delta$ decays exponentially with $n$.
\end{proof}

\textcolor{blue}{To be substantiated: In fact, the result can be generalized beyond binary random variable.}

\subsubsection{Values of the Remote Nodes Conditioned on a Center}
%

Let $\mathcal{R}$ represents the set of remote nodes, which are at least $k$ steps away from a center node $X_c$. Let $m = |\mathcal{R}|$. %

%
%
%
%

There are two special cases of the choice of $X_c$, the root $X_0$ and the tail $X_n$. The reason is that the upstream and the downstream nodes are independent conditioned on $X_c$, so we can always divide the chain into two sub-chains at the center node, calculate the above ratio for each sub-chain and multiply them together for the final answer.  

First we assume the center node $X_c$ is the root.
%
\begin{lemma}{(Value of the Downstream Remote Nodes)}
\begin{equation}\label{eqn:correlation_remote_down}
\frac{\frac{1}{2} - |\Delta|}{\frac{1}{2} + |\Delta|}\leq \frac{P(\XR = x_\calR|X_0 = 0)}{P(\XR = x_\calR|X_0 = 1)} \leq \frac{\frac{1}{2} + |\Delta|}{\frac{1}{2} - |\Delta|}
\end{equation}
where $\Delta = \frac{1}{2} (2p-1)^k$ and $x_\calR$ is any realization of the set of remote nodes $\calR$.
\end{lemma}

\begin{proof}
Let's rename $\XR$ as $\{Y_1, \dots, Y_m\}$, where $Y_j$ depends only on $Y_{j-1}$. And correspondingly we have $\{y_1, \dots, y_m\}$. Then we have

\begin{align*}
&   \sup_{\vec{y}}  \frac{P(\vec{Y} = \vec{y}|X_0 = 0)}{P(\vec{Y} = \vec{y}|X_0 = 0)} \\
=&  \sup_{\vec{y}} \frac{P(Y_1 = y_1|X_0 = 0)\prod_{j=2}^m P(Y_j = y_j|Y_{j-1} = y_{j-1})}{P(Y_1 = y_1|X_0 = 0)\prod_{j=2}^m P(Y_j = y_j|Y_{j-1} = y_{j-1})} \\
=&  \sup_{\vec{y}} \frac{P(Y_1 = y_1|X_0 = 0)}{P(Y_1 = y_1|X_0 = 1)}\\
\leq&\ \frac{\frac{1}{2} + |\Delta|}{\frac{1}{2} - |\Delta|}
\end{align*}

Similarly we can also find the lower bound of the sum of the remote nodes as $\frac{\frac{1}{2} - |\Delta|}{\frac{1}{2} + |\Delta|}$.
\end{proof}

%
%
%
%
%

%
%

%
%
%
%
%
%
%
%
%
%
%

%
%
%
%
%

The same trick can be used again when the center $X_c$ is the tail.

\begin{lemma}{(Value of the Upstream Remote Nodes)}
\begin{equation}\label{eqn:correlation_remote_up}
\left(\frac{\frac{1}{2} - |\Delta|}{\frac{1}{2} + |\Delta|}\right)^2
\leq 
\frac{P(\XR = x_\calR|X_n = 0)}{P(\XR = x_\calR|X_n = 1)} 
\leq
\left(\frac{\frac{1}{2} + |\Delta|}{\frac{1}{2} - |\Delta|}\right)^2
\end{equation}
where $\Delta = \frac{1}{2} (2p-1)^k$ and $x_\calR$ is any realization of the set of remote nodes $\calR$.
\end{lemma}

%
%
%
%
%
%
%
%

\begin{proof}
Similar to the downstream proof.
\end{proof}

%

We immediately observe that the values $\XR$ of the remote nodes itself preserves some privacy without adding any noise, because the ratio in \eqref{eqn:correlation_remote_down} and \eqref{eqn:correlation_remote_up} are naturally bounded. We can always find a large enough privacy-parameter $\delta$ such that it is $\delta$-Pufferfish private.

\textcolor{blue}{Generalization:}
The proof of Lemma 4.4 and 4.5 reveals a potentially useful insight of the correlation decay model, that is, a Markov blanket can be used to upperbound the ratio of the probability conditioned on the target to be protected. 

%

\subsubsection{Putting Together for Pufferfish Privacy}
Now we shall formally give the privacy mechanism to the "genetic-disease-in-a-small-town" problem, where the target to be protected is $X_c$.

Let $X$ be the set of all nodes.

Let $\mathcal{N}$, the set of nodes near the center, be all the nodes not in $\mathcal{R}$, with $|\mathcal{N}| = k$. 

Let $\mathcal{D}$ be the underlying distribution (which fully reflects correlation between nodes), $(X_c = 0, X_c = 1)$ to be the secret pair we are protecting. 

%

%
%
%

%
%
%

%
%
%
%
%
%

%
%

%
%
%
%
%
%

%
%
%
%

Let $\calF(X)$ be 1-Lipschitz, i.e., $|\calF(x_1, \dots, x_i, \dots, x_n) - \calF(x_1, \dots, x_i', \dots, x_n)| \leq 1$ for all $i, x_i, x_i'$.

The mechanism $M$ returns $M(X) = \calF(X) + Z$, where $Z \sim \Lap(k/\lambda)$. 

\begin{theorem}
If $\calF(x_1,\dots,x_n)$ is 1-Lipschitz, then $M$ preserves $\epsilon$-Pufferfish privacy, where $\epsilon = \delta + \lambda$, and $\delta$ is the privacy-parameter of the self-private-preserving sum of the remote nodes set $\mathcal{R}$.
\end{theorem}

\begin{proof}
To simplify the notation we use $\calF(\XR, \XN)$ to represent $\calF(X)$. 

The algorithm M is said to satisfy $\epsilon$-Puffer-fish privacy if for any output $t$,
$$e^{-\epsilon} \leq \frac{p(\calF(\XR, \XN) + Z = t | X_c = 0, \mathcal{D})}{p(\calF(\XR, \XN) + Z = t | X_c = 1, \mathcal{D})}\leq e^\epsilon$$

Factorize the expression to get
\begin{align*}
&   \frac{p(\calF(\XR, \XN) + Z = t | X_c = 0, \mathcal{D})}{p(\calF(\XR, \XN) + Z = t | X_c = 1, \mathcal{D})} \\
=&  \frac{\sum_{\text{all configures }x_\calR} p(\XR=x_\calR | X_c = 0, \calD) p(\calF(\XR, \XN) + Z = t | X_c = 0, \XR=x_\calR, \calD)}{\sum_{\text{all configures }x_\calR} p(\XR=x_\calR | X_c = 1, \calD) p(\calF(\XR, \XN) + Z = t | X_c = 1, \XR=x_\calR, \calD)}
\end{align*}

By the definition of $\delta$,
\begin{align*}
e^{-\delta} \leq
\frac{p(\XR=x_\calR | X_c = 0, \calD)}{p(\XR=x_\calR | X_c = 1, \calD)}
\leq e^\delta
\end{align*}

Also, since $|\calF(x_1, \dots, x_i, \dots, x_n) - \calF(x_1, \dots, x_i', \dots, x_n)| \leq 1$ for all $i$, the noise $Z$ guarantees
\begin{align*}
e^{-\lambda} \leq
\frac{p(\calF(\XR, \XN) + Z = t | X_c = 0, \XR=x_\calR, \calD)}{p(\calF(\XR, \XN) + Z = t | X_c = 1, \XR=x_\calR, \calD)}
\leq e^\lambda
\end{align*}

Therefore, 
$$\epsilon = \delta + \lambda$$
which is a function of the number of near nodes $k$ and the noise distribution parameter $\lambda$.
\end{proof}


%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%


==> fastAlgorithm.tex <==
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

\begin{algorithm}
\caption{\fastAlgo($\epsilon$, $F$, $D$)}
\label{alg:MQM fast}
\begin{algorithmic}
\STATE {Initialize $\sigma_{\max} \gets 0$}
\STATE {$T = |\calX|$}
\STATE {$i = \lfloor \frac{T}{2} \rfloor$}
\WHILE {$i$ has not being explored}
 \STATE {Mark $i$ as explored}
 \STATE {$(a_i, b_i, \sigma_i) \gets \subroutine \left(i, \epsilon\right)$}
 \STATE {$\sigma_{\max}  = \max(\sigma_{\max} , \sigma_i)$}
 \IF {$i-a_i = 0$ and $i+b_i = T+1$}
   \STATE {\textbf{break}}%
 \ELSIF {$i - a_i = 0$}
   \STATE {$i = i+1$}
 \ELSIF {$i + b_i = T+1$}
   \STATE{$i = i-1$}
 \ELSE
   \STATE{\textbf{break}}%
 \ENDIF
\ENDWHILE
\STATE{\textbf{return} $F(D) + \sigma_{\max}\cdot\Lap(1)$}
\end{algorithmic}
\end{algorithm}

